Joint Optimization of Neural Radiance Fields and Continuous Camera Motion from a Monocular Video

Neural Radiance Fields (NeRF) has demonstrated its superior capability to represent 3D geometry but require accurately precomputed camera poses during training. To mitigate this requirement, existing methods jointly optimize camera poses and NeRF often relying on good pose initialisation or depth priors. However, these approaches struggle in challenging scenarios, such as large rotations, as they map each camera to a world coordinate system. We propose a novel method that eliminates prior dependencies by modeling continuous camera motions as time-dependent angular velocity and velocity. Relative motions between cameras are learned first via velocity integration, while camera poses can be obtained by aggregating such relative motions up to a world coordinate system defined at a single time step within the video. Specifically, accurate continuous camera movements are learned through a time-dependent NeRF, which captures local scene geometry and motion by training from neighboring frames for each time step. The learned motions enable fine-tuning the NeRF to represent the full scene geometry. Experiments on Co3D and Scannet show our approach achieves superior camera pose and depth estimation and comparable novel-view synthesis performance compared to state-of-the-art methods. Our code is available at https://github.com/HoangChuongNguyen/cope-nerf.

==> main/3_method_subsection/3_sdf_flow_loss.tex <==

\subsection{SDF and Scene Flow Consistency}
\label{subsec:sdf_scene_consistency} 
\wm{Can this section be merged to to loss function section?} \\
As the camera moves, the observed geometry also changes. This implies that motions of surface points (i.e., scene flows) are tightly coupled with the temporal changes of the observed scene geometry (i.e., SDF flows).
% , which can be represented as the changes in the SDF field along the temporal dimension (i.e., SDF flow $\Delta s$). 
Given a surface point $\mathbf{\tilde{x}}$, the relation between its scene flow $\Delta{\mathbf{\tilde{x}}}$ and SDF flow $\Delta s$ has been studied in \cite{maoneural} through the following expression:
\begin{equation}
    \frac{\partial \phi_g(\mathbf{\tilde{x}}(t))}{\partial t} = -\frac{\partial \phi_g(\mathbf{\tilde{x}}(t))}{\partial \mathbf{\tilde{x}}(t)} \frac{\partial \mathbf{\tilde{x}}(t)}{\partial t} \Leftrightarrow \Delta s = - \mathbf{n}^T \Delta \mathbf{\tilde{x}},
    \label{equa:SDF_flow_relation}
\end{equation}
where $\mathbf{n}$ is the surface normal at $\mathbf{\tilde{x}}$. In our method, we incorporate this relation as a loss function  enforcing the consistency between the geometry inferred from the SDF flow and that inferred from scene flow:
\begin{equation}
     \mathcal{L}_{flow} = |\Delta s_t + \mathbf{n}_t^T \Delta \mathbf{\tilde{x}}_t| 
    \label{equa:L_flow}
\end{equation}
By leveraging the time-dependent NeRF, the SDF flow $\Delta s_t$ and the normal $\mathbf{n}_t$ can be achieved using PyTorch automatic differentiation \cite{paszke2017automatic}: 
\begin{equation}
    \Delta s_t = \frac{ \partial \phi^t_g(\mathbf{\tilde{x}}_t, t) } {\partial t}, \quad     \mathbf{n}_t = \frac{ \partial \phi^t_g(\mathbf{\tilde{x}}_t, t) } {\partial \mathbf{\tilde{x}}_t }. 
\end{equation}
While \cite{maoneural} also makes use of the SDF and SDF flows, our approach for obtaining these information are more efficient because we can avoid the time-consuming SDF flows integration. Regarding the scene flow $\Delta \mathbf{\tilde{x}}_t$, it can be derived from the predicted camera motion:
\begin{equation}
    \Delta \mathbf{\tilde{x}}_t = -(\boldsymbol{\omega}_t \times \mathbf{\tilde{x}}_t + \mathbf{v}_t).
\end{equation}
Since Equa. \ref{equa:SDF_flow_relation} is only valid for surface points, it is important to minimize the impact of non-surface points in $\mathcal{L}_{flow}$. Thus, we measure the influence of each 3D point $\mathbf{x}_t^i$ using its rendering weight $\alpha^i_t$ (see Equa. \ref{equa:render_3dpoint_weight}). As a result, our final $\mathcal{L}_{flow}$ is:
\begin{equation*}
    \mathcal{L}_{flow} = \frac{1}{|\Omega|}\sum_{r \in \Omega} \sum_{i=1}^{N} \text{SG}(\alpha_t^i) |\Delta s_t^i + (\mathbf{n}_t^i)^T \Delta \mathbf{x}^i_t(r) | .
\end{equation*}
We use $\text{SG}(.)$ to represent the stop gradient operation. This loss function provides learning signals to improve both NeRF's geometric representation (via $\Delta s_t^i$ and $\mathbf{n}_t^i$)  and camera motions (via $\boldsymbol{\omega}_t$ and $\mathbf{v}_t$). 


==> main/4_experiments_subsection/limitations.tex <==

\subsection{Limitations}

Our method struggles in regions with view-variant colors or lack of distinct features as they provide insufficient or misleading visual cues for learning the scene geometry. Fig. \ref{fig:limitation} (left) illustrates an example where it produces inaccurate depths for reflective surfaces (green boxes) and low-texture regions (purple box). However, since NeRF is trained to model view-dependent colors, we observe that our method can occasionally capture the properties of such surfaces (see Fig. \ref{fig:limitation} - right), although this is not consistently reliable. On the other hand, the challenges in low-texture regions can be alleviated by exploiting the depth smoothness prior.




==> main/4_experiments_subsection/results/image.tex <==
% \usepackage{rotating}
% \usepackage{tabularray}
\begin{table*}
\centering
\small
\begin{tblr}{
  colsep  = 3.75pt,
  rowsep  = 1pt,
  column{2} = {c},
  column{3} = {c},
  column{4} = {c},
  column{5} = {c},
  column{7} = {c},
  column{8} = {c},
  column{9} = {c},
  column{11} = {c},
  column{12} = {c},
  column{13} = {c},
  column{15} = {c},
  column{16} = {c},
  cell{1}{1} = {r=2}{},
  cell{1}{2} = {r=2}{},
  cell{1}{3} = {c=3}{},
  cell{1}{7} = {c=3}{},
  cell{1}{11} = {c=3}{},
  cell{1}{15} = {c=3}{},
  cell{2}{14} = {c},
  cell{3}{1} = {r=4}{},
  cell{3}{14} = {c},
  cell{3}{17} = {c},
  cell{4}{14} = {c},
  cell{4}{17} = {c},
  cell{5}{14} = {c},
  cell{5}{17} = {c},
  cell{6}{14} = {c},
  cell{6}{17} = {c},
  cell{7}{1} = {r=5}{},
  cell{7}{17} = {c},
  cell{8}{17} = {c},
  cell{9}{17} = {c},
  cell{10}{17} = {c},
  cell{11}{17} = {c},
  hline{1,3,7,12} = {-}{},
  hline{2} = {3-5,7-9,11-13,15-17}{},
}
 & Scenes     & Ours                  &                       &                          &  & NeRFmm$^{\dagger\dagger}$ \cite{wang2021nerf}        &               &                &  & NoPe-NeRF$^{*\dagger}$ (D) \cite{bian2023nope} &               &                &  & CF3DGS$^{\dagger*}$ (D) \cite{fu2023colmapfree}     &               &                \\
                                      &            & $\text{PSNR}\uparrow$ & $\text{SSIM}\uparrow$ & $\text{LPIPS}\downarrow$ &  & $\text{PSNR}$ & $\text{SSIM}$ & $\text{LPIPS}$ &  & $\text{PSNR}$ & $\text{SSIM}$ & $\text{LPIPS}$ &  & $\text{PSNR}$  & $\text{SSIM}$ & $\text{LPIPS}$ \\
\begin{sideways}Scannet\end{sideways} & 0079       & \textbf{35.52}        & \textbf{0.92}         & \underline{0.20}             &  & 32.06         & \underline{0.85}  & 0.33           &  & 32.47         & 0.84          & 0.41           &  & \underline{33.91}  & \textbf{0.92} & \textbf{0.16}  \\
                                      & 0418       & \textbf{34.53}                      & \textbf{0.92}                      & \underline{0.29}                         &   & 30.92              & 0.78              & 0.30               &  & 31.33         & 0.79          & 0.34           &  & 32.56          & 0.90          & \textbf{0.20}           \\
                                      & 0301       & \textbf{32.06}        & \textbf{0.88}         & \underline{0.22}             &  & 30.10         & \underline{0.83}  & 0.29           &  & 29.83         & 0.77          & 0.36           &  & \underline{31.09}  & \textbf{0.88} & \textbf{0.20}  \\
                                      & 0431       & \textbf{34.25}        & \textbf{0.93}         & \underline{0.25}             &  & 32.94         & 0.90          & 0.31           &  & \underline{33.83} & \underline{0.91}  & 0.39           &  & 31.02          & 0.90          & \textbf{0.22}  \\
\begin{sideways}Co3D\end{sideways}    & Bench      & \textbf{26.36}        & \underline{0.68}          & \underline{0.40}             &  & 23.31         & 0.58          & 0.55           &  & 24.32         & 0.60          & 0.52           &  & \underline{26.21}  & \textbf{0.73} & \textbf{0.32}  \\
                                      & Skateboard & \textbf{30.93}        & \textbf{0.87}         & \underline{0.32}             &  & 23.10         & 0.75          & 0.47           &  & 26.22         & 0.80          & 0.42           &  & \underline{27.24}  & \underline{0.85}  & \textbf{0.30}  \\
                                      & Plant      & \underline{26.53}         & \underline{0.77}          & \underline{0.41}             &  & 22.26         & 0.68          & 0.52           &  & 23.79         & 0.71          & 0.48           &  & \textbf{29.69} & \textbf{0.89} & \textbf{0.29}  \\
                                      & Hydrant    & \underline{20.60}         & \underline{0.51}          & \underline{0.44}                     &  & 19.11         & 0.41          & 0.59           &  & 19.82         & 0.42          & 0.57           &  & \textbf{22.14} & \textbf{0.64} & \textbf{0.34}  \\
                                      & Teddy      & \textbf{33.04}        & \textbf{0.89}         & \textbf{0.20}            &  & 27.87         & 0.77          & 0.42           &  & \underline{29.40}         & 0.80          & 0.38           &  & 27.75          & \underline{0.86}  & \textbf{0.20}        
\end{tblr}
\caption{Image evaluation. Our approach significantly outperforms prior NeRF-based methods and is on par with CF3DGS.}
\label{tab:result_image}
\end{table*}


==> main/4_experiments_subsection/results/limitation_vis.tex <==
\begin{figure}
    \centering
    \setlength{\tabcolsep}{3pt}
    \renewcommand{\arraystretch}{0.5}
    \begin{tabular}{c|c}
        % First row
        \begin{subfigure}[b]{0.32\linewidth}
            \centering
            \caption*{Ground-truth image}
            \includegraphics[width=\linewidth]{figures/limitation_visualization/gt_image.png}
        \end{subfigure} 
        \begin{subfigure}[b]{0.32\linewidth}
            \centering
            \caption*{Ground-truth depth}
            \includegraphics[width=\linewidth]{figures/limitation_visualization/gt_depth.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.32\linewidth}
            \centering
            \caption*{Ground-truth image}
            \includegraphics[width=\linewidth]{figures/limitation_visualization/chruch_image.png}
        \end{subfigure} \\

        % Second row
        \begin{subfigure}[b]{0.32\linewidth}
            \centering
            \includegraphics[width=\linewidth]{figures/limitation_visualization/error_map.png}
            \caption*{Depth errors map}
        \end{subfigure} 
        \begin{subfigure}[b]{0.32\linewidth}
            \centering
            \includegraphics[width=\linewidth]{figures/limitation_visualization/my_depth.png}
            \caption*{Our rendered depth}
        \end{subfigure} &
        \begin{subfigure}[b]{0.32\linewidth}
            \centering
            \includegraphics[width=\linewidth]{figures/limitation_visualization/chruch_depth.png}
            \caption*{Our rendered depth}
        \end{subfigure}
    \end{tabular}
    
    \caption{\textbf{Left}: Limitations of our method in \textcolor{ForestGreen}{reflective} and \textcolor{purple}{low-texture} regions. Red areas in the error map indicate high error. \textbf{Right}: Our method can occasionally produce correct geometry for reflective regions.}
    % , although this is not always guaranteed.}
    \label{fig:limitation}
\end{figure}


==> main/4_experiments_subsection/results/pose.tex <==
\begin{table*}
\centering
\small
\begin{tblr}{
  colsep  = 4.5pt,
  rowsep  = 1pt,
  column{2} = {c},
  column{3} = {c},
  column{4} = {c},
  column{5} = {c},
  column{7} = {c},
  column{8} = {c},
  column{9} = {c},
  column{11} = {c},
  column{12} = {c},
  column{13} = {c},
  column{15} = {c},
  column{16} = {c},
  cell{1}{1} = {r=2}{},
  cell{1}{2} = {r=2}{},
  cell{1}{3} = {c=3}{},
  cell{1}{7} = {c=3}{},
  cell{1}{11} = {c=3}{},
  cell{1}{15} = {c=3}{},
  cell{2}{14} = {c},
  cell{3}{1} = {r=4}{},
  cell{3}{14} = {c},
  cell{3}{17} = {c},
  cell{4}{14} = {c},
  cell{4}{17} = {c},
  cell{5}{14} = {c},
  cell{5}{17} = {c},
  cell{6}{14} = {c},
  cell{6}{17} = {c},
  cell{7}{1} = {r=5}{},
  cell{7}{17} = {c},
  cell{8}{17} = {c},
  cell{9}{17} = {c},
  cell{10}{17} = {c},
  cell{11}{17} = {c},
  hline{1,3,7,12} = {-}{},
  hline{2} = {3-5,7-9,11-13,15-17}{},
}
                   & Scenes     & Ours                     &                          &                        &  & NeRFmm$^{\dagger\dagger}$ \cite{wang2021nerf}         &                &              &  & NoPe-NeRF$^{*\dagger}$ (D) \cite{bian2023nope}  &                &               &  & CF3DGS$^{\dagger*}$ (D) \cite{fu2023colmapfree}     &                &               \\
                                      &            & $\text{RPE}_t\downarrow$ & $\text{RPE}_r\downarrow$ & $\text{ATE}\downarrow$ &  & $\text{RPE}_t$ & $\text{RPE}_r$ & $\text{ATE}$ &  & $\text{RPE}_t$ & $\text{RPE}_r$ & $\text{ATE}$  &  & $\text{RPE}_t$ & $\text{RPE}_r$ & $\text{ATE}$  \\
\begin{sideways}Scannet\end{sideways} & 0079       & \textbf{0.664}           & \textbf{0.182}           & \textbf{0.013}         &  & 3.312          & 0.801          & 0.151        &  & 0.752          & 0.204          & 0.023         &  & \underline{0.673}  & \underline{0.190}  & \underline{0.015} \\
                                      & 0418       & \textbf{0.401}	                         & \textbf{0.119}	                         & \textbf{0.015}                       &  & 1.428          & 0.396          & 0.016        &  & \underline{0.455}  & \textbf{0.119}  & \textbf{0.015} &  & 0.529          & 0.131          & 0.019         \\
                                      & 0301       & \textbf{0.367}           & \textbf{0.117}           & \textbf{0.009}         &  & 1.852          & 0.591          & 0.296        &  & 0.399          & 0.123          & \underline{0.013} &  & \underline{0.393}  & \underline{0.118}  & 0.015         \\
                                      & 0431       & \textbf{1.097}           & \textbf{0.223}           & \textbf{0.042}         &  & 6.661          & 0.574          & 0.475        &  & 1.625          & 0.274          & 0.069         &  & \underline{1.301}  & \underline{0.269}  & \underline{0.064} \\
\begin{sideways}Co3D\end{sideways}    & Bench      & \textbf{0.013}           & \textbf{0.037}           & \textbf{0.001}         &  & 0.562          & 3.508          & 0.039        &  & 0.301          & 1.925          & 0.053         &  & \underline{0.110}  & \underline{0.424}  & \underline{0.014} \\
                                      & Skateboard & \textbf{0.024}           & \textbf{0.063}           & \textbf{0.001}         &  & 0.702          & 2.794          & 0.057        &  & 0.421          & 1.883          & 0.048         &  & \underline{0.239}  & \underline{0.472}  & \underline{0.017} \\
                                      & Plant      & \textbf{0.014}           & \textbf{0.062}           & \textbf{0.002}         &  & 0.650          & 2.557          & 0.059        &  & 0.305          & 1.587          & 0.047         &  & \underline{0.140}  & \underline{0.401}  & \underline{0.021} \\
                                      & Hydrant    & \textbf{0.010}           & \textbf{0.027}           & \textbf{0.001}         &  & 0.497          & 2.556          & 0.063        &  & 0.337          & 1.557          & 0.060         &  & \underline{0.094}  & \underline{0.360}  & \underline{0.008} \\
                                      & Teddy      & \textbf{0.053}           & \textbf{0.129}           & \textbf{0.004}         &  & 0.588          & 3.025          & 0.049        &  & \underline{0.286}  & 1.295          & 0.040         &  & 0.505          & \underline{0.211}  & \underline{0.009}     
\end{tblr}
\caption{Pose evaluation. Our method achieves the lowest pose errors in all scenes.}
\label{tab:result_pose}
\end{table*}
